GraPPa: Grammar-Augmented Pre-Training for Table Semantic Parsing

We present GraPPa, an effective pre-training approach for table semantic parsing that learns a compositional inductive bias in the joint representations of textual and tabular data. We construct synthetic question-SQL pairs over high-quality tables via a synchronous context-free grammar (SCFG) induced from existing text-to-SQL datasets. We pre-train our model on the synthetic data using a novel text-schema linking objective that predicts the syntactic role of a table field in the SQL for each question-SQL pair. To maintain the model's ability to represent real-world data, we also include masked language modeling (MLM) over several existing table-and-language datasets to regularize the pre-training process. On four popular fully supervised and weakly supervised table semantic parsing benchmarks, GraPPa significantly outperforms RoBERTa-large as the feature representation layers and establishes new state-of-the-art results on all of them.

==> sections/problem.tex <==
\section{Problem Definition}
\vic{define table semantic parsing, both fully and weakly supervised, formally and succinctly}

==> tables/result_spider.tex <==
\begin{table}[t]
\centering
\scalebox{0.78}{
\begin{tabular}{lcc}
\Xhline{2\arrayrulewidth}
Models & Dev. & Test \\ \hline
Global-GNN \cite{Bogin2019GlobalRO} & 52.7 & 47.4 \\
EditSQL $w.$ BERT \cite{zhang19} & 57.6 & 53.4\\
IRNet $w.$ BERT \cite{Guo2019TowardsCT} & 61.9 & 54.7\\
RYANSQL $w.$ BERT \cite{Choi2020RYANSQLRA} & 70.6 & 60.6\\
TranX $w.$ TaBERT \cite{yin-etal-2020-tabert} & 64.5 & - \\
\Xhline{2\arrayrulewidth}
RAT-SQL  \cite{wang2019} & 62.7 & 57.2 \\
\hspace{0.1cm} $w.$ BERT-large & 69.7 & 65.6 \\
\hspace{0.1cm} $w.$ RoBERTa-large & 69.6 %\pm 0.17 
& - \\
\hspace{0.1cm} $w.$ \tablebert{} (MLM) & 71.1 %\pm 0.17 
& - \\
\hspace{0.1cm} $w.$ \tablebert{} (SSP) & \bf{73.6} %\pm 0.20 
& 67.7 \\
\hspace{0.1cm} $w.$ \tablebert{} (MLM+SSP) & 73.4 %\pm 0.80 
& \bf{69.6} \\
\Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{Performance on \textsc{Spider}. We use RAT-SQL + BERT \cite{wang2019} as our base model. We run each model three times by varying random seeds, and the average scores are shown.}
\vspace{-3mm}
\label{tab:res_spider}
\end{table}

==> tables/result_wikisql.tex <==
\begin{table}[t!]
\centering
\small
\scalebox{0.94}{
\begin{tabular}{lcc}
\Xhline{2\arrayrulewidth}
Models & Dev. & Test \\\hline
\citet{Zhong2017} & 60.8 & 59.4 \\ 
\citet{Xu2017} & 69.8 & 68.0 \\ 
\citet{Yu18} & 74.5 & 73.5 \\
\citet{dong18} & 79.0 & 78.5 \\ 
\citet{shi2018incsql} & 84.0 & 83.7 \\
\citet{Hwang2019ACE} & 87.2 & 86.2 \\
\citet{He2019XSQLRS} & 89.5 & 88.7 \\
\citet{lyu2020hybrid} & 89.1 & 89.2 \\
\Xhline{2\arrayrulewidth}
\citet{Guo2019} & 90.3 & 89.2 \\
\hspace{0.1cm} $w.$ RoBERTa-large & 91.2 & 90.6 \\
\hspace{0.1cm} $w.$ \tablebert{} (MLM) & 91.4 & 90.7 \\
\hspace{0.1cm} $w.$ \tablebert{} (SSP) & 91.2 & 90.7 \\
\hspace{0.1cm} $w.$ \tablebert{} (MLM+SSP) & 91.2 & \bf{90.8} \\
\hline
\hspace{0.1cm} $w.$ RoBERTa-large (10k) & 79.6 & 79.2 \\
\hspace{0.1cm} $w.$ \tablebert{} (MLM+SSP) (10k) & \bf{82.3(+2.7)} & \bf{82.2(+3.0)} \\
\Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{Performance on fully-sup. \textsc{WikiSQL}. All results are on execution accuracy without execution-guided decoding. We run each model twice and the results are the same. Results on models trained on 10k (18\%) \textsc{WikiSQL} examples are shown at the bottom.}
\label{tab:res_wikisql}
\end{table}


\hide{
\begin{table}[Ht!]
\centering
\small
\scalebox{0.96}{
\begin{tabular}{lccc}
\Xhline{2\arrayrulewidth}
$\mathbb{|L|}$ & \roberta{} & \tablebert{} \\\hline
10,000 & 62.7 & \bf{69.7} (+7.0) \\ %35.1
30,000 & 80.2  & \bf{81.6} (+1.4) \\ %5.2
56,355 (all) & 82.1 & \bf{82.8} (+0.7) \\ %4.8
\Xhline{2\arrayrulewidth}
\multicolumn{3}{l}{Models} & $Acc._{lf}$ \\\hline
\multicolumn{3}{l}{Coarse2Fine \cite{dong18}} & 72.5 \\
\multicolumn{3}{l}{SQLova \cite{Hwang2019ACE}} & 81.6 \\
\multicolumn{3}{l}{X-SQL \cite{He2019XSQLRS}} & \bf{83.8} \\
\Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{Performance on fully-sup. \textsc{WikiSQL} w.r.t. the size of labeled training data $\mathbb{|L|}$ (top). All models on the top table use SQLova \cite{Hwang2019ACE} as a base model. Also, we show results of previous methods (bottom). All results are in logic form accuracy ($Acc._{lf}$) on the development set. $^*$SQLova with RoBERTa outperforms with BERT.}
\vspace{-3mm}
\label{tab:res_wikisql}
\end{table}
}

==> tables/result_wikitable.tex <==
\begin{table}[t]
\centering
\small
\scalebox{0.94}{
\begin{tabular}{lcc}
\Xhline{2\arrayrulewidth}
Models & Dev. & Test \\\hline
\citet{pasupat2015compositional} & 37.0 & 37.1 \\ 
\citet{Neelakantan2016LearningAN} & 34.1 & 34.2 \\ 
\citet{Haug2017NeuralMR} & - & 34.8 \\ 
\citet{Zhang2017MacroGA} & 40.4 & 43.7 \\ 
\citet{Liang2018MemoryAP} & 42.3 & 43.1 \\ 
\citet{Dasigi2019IterativeSF} & 42.1 & 43.9 \\ 
\citet{Agarwal2019LearningTG} & 43.2 & 44.1 \\ 
\citet{herzig2020tapas} & - &48.8 \\
\citet{yin2020tabert} & 52.2 & 51.8 \\
\Xhline{2\arrayrulewidth}
\citet{wang2019} & 43.7 & 44.5 \\
% \hspace{0.1cm} $w.$ RoBERTa & 48.6 (+4.9) & 49.2 (+4.7) \\
% \hspace{0.1cm} $w.$ TableBERT & 49.3 (+5.6) & 50.5 (+6.0) \\
% \hspace{0.1cm} $w.$ TableBERT $f.t.$ Spider & 49.1 (+5.4) & 50.2 (+5.7) \\
% \hspace{0.1cm} $w.$ TableBERT $f.t.$ WikiSQL & \bf{50.3 (+6.6)} & \bf{50.7 (+6.2)} \\
% \hline
\hspace{0.1cm} $w.$ RoBERTa-large & 50.7(+7.0) & 50.9(+6.4) \\
\hspace{0.1cm} $w.$ \tablebert{} (MLM) & 51.5(+7.8) & 51.7(+7.2) \\
\hspace{0.1cm} $w.$ \tablebert{} (SSP) & 51.2(+7.5) & 51.1(+6.6) \\
\hspace{0.1cm} $w.$ \tablebert{} (MLM+SSP) & \textbf{51.9(+8.2)} & \textbf{52.7(+8.2)} \\

\hline

\hspace{0.1cm} $w.$ RoBERTa-large $\times$10\% & 37.3 & 38.1 \\
\hspace{0.1cm} $w.$ \tablebert{} (MLM+SSP) $\times$10\% & \textbf{40.4(+3.1)} & \textbf{42.0(+3.9)}\\

\Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{Performance on \textsc{WikiTableQuestions}. We use \citet{wang2019} as a base model. Results trained on 10\% of the data are shown at the bottom.
% $f.t.$ stands for fine tuning on.
}
% \drr{the caption says "fine tuning on." and doesn't end there}
%\vspace{-2mm}
\label{tab:res_wikitable}
\end{table}

==> tables/result_wsp_wikisql.tex <==
\begin{table}[t]
\centering
\scalebox{0.78}{
\begin{tabular}{lcc}
\Xhline{2\arrayrulewidth}
Models & Dev. & Test \\\hline
\citet{Liang2018MemoryAP} & 72.2 & 72.1 \\ 
\citet{Agarwal2019LearningTG} & 74.9 & 74.8 \\
\citet{min2019discrete} & 84.4 & 83.9 \\
\citet{herzig2020tapas} & 85.1 & 83.6 \\
\Xhline{1\arrayrulewidth}
\citet{wang2019} & 79.4 & 79.3 \\
\hspace{0.1cm} $w.$ RoBERTa-large & 82.3 (+2.9) & 82.3 (+3.0) \\
\hspace{0.1cm} $w.$ \tablebert{} (MLM) & 83.3 (+3.9) & 83.5 (+4.2) \\
\hspace{0.1cm} $w.$ \tablebert{} (SSP) & 83.5(+4.1) & 83.7 (+4.4) \\
\hspace{0.1cm} $w.$ \tablebert{} (MLM+SSP) & \bf{85.9} (+6.5) & \bf{84.7} (+5.4) \\
%\hspace{0.1cm} $w.$ Ours $f.t.$ Spider & 85.7 (+6.3) & 83.3 (+4.0) \\
%\hspace{0.1cm} $w.$ Ours $f.t.$ WikiSQL & 85.8 (+6.3) & \bf{85.6 (+6.3)} \\
\Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{Performance on weakly-sup. \textsc{WikiSQL}. We use \citet{wang2019} as our base model. 
% $f.t.$ stands for fine tuning on
% \vic{caption is broken; can cut strong supervised model results}
}
\label{tab:res_wsp_wikisql}
\vspace{-1mm}
\end{table}
